The Impact of Technical Domain Expertise on Search Behavior and Task Outcome

Domain expertise is regarded as one of the key factors impacting search success: experts are known to write more effective queries, to select the right results on the result page, and to find answers satisfying their information needs. Search transaction logs play the crucial role in the result ranking. Yet despite the variety in expertise levels of users, all prior interactions are treated alike, suggesting that weighting in expertise can improve the ranking for informational tasks. The main aim of this paper is to investigate the impact of high levels of technical domain expertise on both search behavior and task outcome. We conduct an online user study with searchers proficient in programming languages. We focus on Java and Javascript, yet we believe that our study and results are applicable for other expertise-sensitive search tasks. The main findings are three-fold: First, we constructed expertise tests that effectively measure technical domain expertise and correlate well with the self-reported expertise. Second, we showed that there is a clear position bias, but technical domain experts were less affected by position bias. Third, we found that general expertise helped finding the correct answers, but the domain experts were more successful as they managed to detect better answers. Our work is using explicit tests to determine user expertise levels, which is an important step toward fully automatic detection of expertise levels based on interaction behavior. A deeper understanding of the impact of expertise on search behavior and task outcome can enable more effective use of expert behavior in search logs - essentially make everyone search as an expert.

==> background.tex <==
\todo[Maybe merge into intro -- if only to save space -- has lot's of the old focus -- and is way too long...  Must include more studies on "expertise"...]

% Literature suggestions:
% 
% [09-02-15 18:57:35] Jaap Kamps: That's the spirit -- no problem -- we'll cite a few related studies...  E.g., there's the work of CLUES, in particular Ryen and Sue on expertise,
% Characterizing the Influence of Domain Expertise on Web Search Behavior
% http://research.microsoft.com/apps/pubs/default.aspx?id=79630
%  with some other spin-offs like the papers using reading level to guess expertise levels,
% Personalizing web search results by reading level, CIKM'11
% http://dl.acm.org/citation.cfm?id=2063639
% 
% Knowledge effects on document selection in search results pages, SIGIR'11
% http://dl.acm.org/citation.cfm?id=2010128
%
% A Study of Querying Behaviour of Expert and Non-expert Users of Biomedical Search Systems, ADCS'14
% http://dl.acm.org/citation.cfm?id=2682871
%
% Are self-assessments reliable indicators of topic knowledge? ASIST'10
% http://dl.acm.org/citation.cfm?id=1920375
%
% Predicting user interests from contextual information, SIGIR'09
% http://dl.acm.org/citation.cfm?id=1572005
%
% Large-scale analysis of individual and task differences in search result page examination strategies, WSDM'12
% http://dl.acm.org/citation.cfm?id=2124341
%
% On domain expertise-based roles in collaborative information retrieval, IPM'14
% http://dl.acm.org/citation.cfm?id=2657829
% 
% And of course some of our own stuff :)
% 
% Search log analysis of user stereotypes, information seeking behavior, and contextual evaluation, IIiX'10
% http://humanities.uva.nl/~kamps/publications/2010/zhan:sear10b.pdf
% 
% Various user studies, including: RAIO'10; DIR'10/ECA'10 (just ignore). 

\begin{comment}
Literature suggestions from Nik:

%Using expert users to rank results for novice users
Position bias + taking time into account: http://dl.acm.org/citation.cfm?id=2348300&CFID=459881203&CFTOKEN=83626747
Popular destinations by R. White (your MSR mentor): http://dl.acm.org/citation.cfm?id=1277771. They try to see what pages people end up with and then try to rank those pages higher (reminds me the idea/motivation in the paper)
Ask crowdworkers to find short answers to factoid questions and then show these answers on the search page (kind of usages of expertise of crowd to find relevant pages that might save efforts for novice users): http://hci.stanford.edu/publications/2012/tailanswers/tailanswers-chi2012.pdf
Information credibility- "Levels of experience and how respondents perceived the credibility of information were related to whether they verified information. This study explores the social relevance of the findings and discusses them in terms of theoretical knowledge of advanced communication technologies." http://jmq.sagepub.com/content/77/3/515.abstract


%Novice vs. Experts searching for information
An empirical comparison of the usability for novice and expert searchers of a textual and a graphic interface to an art-resource database https://www.ischool.utexas.edu/~adillon/Journals/JODI-final-pics_files/empirical%20comparison.htm
Differences between Novice and Experienced Users in Searching Information on the World Wide Web file:///C:/Users/Spirinus/Downloads/Lazonder%20et%20al%20JASIS%202000.pdf
Searching on the web two types of expertise: http://dl.acm.org/citation.cfm?id=312737&dl=ACM&coll=DL&CFID=459881203&CFTOKEN=83626747
Web search behavior of Internet experts and newbies: http://dl.acm.org/citation.cfm?id=347319.346311
http://dl.acm.org/citation.cfm?id=1357062&CFID=459881203&CFTOKEN=83626747 Knowledge in the head and on the web: using topic expertise to aid search
http://dl.acm.org/citation.cfm?id=1646407&CFID=459881203&CFTOKEN=83626747 The role of expertise in aiding video search
http://dl.acm.org/citation.cfm?id=1498819&CFID=459881203&CFTOKEN=83626747 Characterizing the influence of domain expertise on web search behavior
Hsieh-Yee, I. (1993). Effects of search experience and subject knowledge on the search tactics of novice and experienced searchers. JASIST, 44(3), 161--174.
Marchionini, G., Lin, X. & Dwiggins, S. (1990). Effects of search and subject expertise on information seeking in a hypertext environment. Proc. ASIS, 129--142.
The effects of topic familiarity on information search behavior http://dl.acm.org/citation.cfm?id=544232&CFID=459881203&CFTOKEN=83626747
http://dl.acm.org/citation.cfm?id=544232&CFID=459881203&CFTOKEN=83626747 Factors affecting the selection of search tactics: Tasks, knowledge, process, and systems
http://dl.acm.org/citation.cfm?id=1277787&CFID=459881203&CFTOKEN=83626747 Investigating the querying and browsing behavior of advanced search engine users
http://dl.acm.org/citation.cfm?id=1124171&CFID=459881203&CFTOKEN=83626747 Best practices and future visions for search user interfaces
User characteristics for overcoming bias and intrigue in travel searches http://dl.acm.org/citation.cfm?id=1359770&CFID=459881203&CFTOKEN=83626747
http://dl.acm.org/citation.cfm?id=1351376&CFID=459881203&CFTOKEN=83626747 Web search strategies: The influence of Web experience and task type
http://dl.acm.org/citation.cfm?id=1458160&CFID=459881203&CFTOKEN=83626747 How evaluator domain expertise affects search result relevance judgments
\end{comment}



\textbf{Success in web search}.\emph{However what can we interpret from clicks?} 
Should we say that user click on page is 100\% success and remains? Or user did not have knowledge about the topic he has asked and he is trying to find an right answer? The question about quality of information in Web still remains.
Nevertheless, the evaluation of ranking quality can be really tricky. Originally, user click was interpret as `success', more clicks for the pair \emph{\{Query $Q$, Document $D$\}} we have is better so then most popular page for query $Q$ would be pushed to top-ranked results. The wisdom of the crowd provides us right result.
However, \citet{ageev_sigir_2011} proposed flexible and general informational search success model for
in-depth analysis of search success which was tested based on game-like infrastructure for crowdsourcing search behaviour studies, specifically targeted towards capturing and evaluating successful search strategies on informational tasks with known intent. 

\citep{White_wsdm_2009} proposed strategies to find out users' expertise.

\textbf{User Profiles}. On the other hand, user activity is tracked by publishers and third parties through browser cookies that uniquely identify the user visits to web sites. A variety of different actions are associated with each user as web page visits, search queries, etc. They are distilled into a compact description of the \emph{user profiles}. Survey of user profile generation can be found in~\citep{Gauch_2007}. The user profiling is active area of research due to complications of user behaviour. E.g. \citet{Low_2011} proposed scalable method to capture both the user's long term and short term interests that was specifically designed to satisfy need of behavioural targeting.


Users have different level of authority in different topics and their knowledge influenced the decision they make. If you have some knowledge about `java programming' it would be easy for you to find an answer and verify it because you act as en expert in the field. In this paper we trying to find an answer to question how prior user knowledge influences their clicking behaviour and how can we utilise this bias to improve \emph{quality} of ranking. 



%\begin{figure}[h!]
%\center{\includegraphics[width=0.5\textwidth]{pictures/approach_diag.pdf}}
%\caption{An approach of users' clicks verification.}
%\label{fig:approach}
%\end{figure}

